Multilingual Translation via Grafting Pre-trained Language Models

Can pre-trained BERT for one language and GPT for another be glued together to translate texts? Self-supervised training using only monolingual data has led to the success of pre-trained (masked) language models in many NLP tasks. However, directly connecting BERT as an encoder and GPT as a decoder can be challenging in machine translation, for GPT-like models lack a cross-attention component that is needed in seq2seq decoders. In this paper, we propose Graformer to graft separately pre-trained (masked) language models for machine translation. With monolingual data for pre-training and parallel data for grafting training, we maximally take advantage of the usage of both types of data. Experiments on 60 directions show that our method achieves average improvements of 5.8 BLEU in x2en and 2.9 BLEU in en2x directions comparing with the multilingual Transformer of the same size.

==> 010intro_v1.tex <==

Multilingual neural machine translation (MNMT) has recently become an important research field for the deployment efficiency and transfer learning for low-resource language pairs~\cite{aharoni2019massively}. Most related works follow~\newcite{johnson2017google} and train all language pairs together. It is proved that such mixed training can significantly boost the performance of low-resource pairs~\cite{arivazhagan2019massively}. 
The most straightforward training paradigm of MNMT is feeding parallel data of multiple language pairs. However, the utilization of monolingual data has only been preliminarily explored. Since the scale of monolingual data is tens or even hundreds times of the parallel one, how to leverage monolingual data into MNMT requires much attention. There exists three categories of similar attempts, as are in Figure~\ref{fig:mono}. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/mono.pdf}
    \caption{Recent works using monolingual data on multilingual neural machine translation.}
    \label{fig:mono}
\end{figure}


The first one is incorporating back translation (BT)~\cite{sennrich2016improving,edunov2018understanding} into MNMT~\cite{zhang2020improving,wang2020multi}. For normal NMT, the synthetic data can be easily generated by BT. However, for MNMT, back translation is tremendously costly, reaching to $O(n)$, or even $O(n^2)$ in the non English-Centric scene, let alone iterative methods~\cite{hoang2018iterative}. 
The second one is taking advantage of multi-task learning (MTL)~\cite{caruana1997multitask}. Generally, the training is synchronously supervised by translation and other NLU or NLG tasks~\cite{siddhant2020leveraging,wang2020multi}, making the monolingual data utilized conveniently. The last one is making use of monolingual data in the pre-training stage. Many recent studies have proven the effect of utilizing pre-trained models for NMT~\cite{yang2020towards,zhu2020incorporating}. As for MNMT, based on the specific approach, related works can be further divided into two types: \textit{United Style} and \textit{Assembled Style}.

For \textit{United Style}, \newcite{tang2020multilingual} pre-train a single united sequence-to-sequence model and then load the parameters in the initialization of tuning. Due to the model architecture consistency, the pre-trained sequence model can significantly boost the performance. However, the pre-trained object is usually a variant of auto-encoding~\cite{song2019mass,liu2020multilingual}, which is different from the downstream translation object and may not achieve adequate improvements~\cite{lin2020pre}. Meanwhile, overall tuning may also raise the problem of "catastrophic forgetting" that the pre-trained language knowledge gradually fades away~\cite{goodfellow2013empirical,yang2020towards}.
For \textit{Assembled Style}, \newcite{rothe2020leveraging,ma2020xlm} pre-train a BERT-like encoder~\cite{devlin2019bert} and a GPT-like decoder~\cite{radford2018improving} independently and then assemble them in the fine-tuning translation model. However, mismatches still exist. The translation model has "cross-attention" that links to the encoder while pre-trained models have none. Even though some fixing methods are adopted~\cite{guo2020incorporating}, the original architecture of the pre-trained decoder is still transformed, resulting in the usage limitation of the elaborately trained decoder.

In this paper, we mainly focus on the pre-trained route, trying to extend the \textit{Assembled Style}, specifically. The most crucial drawback of this style is the discrepancy between upstream and downstream. Generally, the cross-attention layer injected in BERT or GPT during the tuning stage  breaks the original structure. The adjusted architecture may make the pre-trained model deteriorates. Therefore, the main target is to link the generation model to the source side and maintain the invariability of the pre-trained models at the same time. 

Therefore, we propose an independent connective structure to solve this problem. Firstly, we pre-train a multilingual BERT and multilingual GPT like previous works. Then we stack a bridge module upon the pre-trained models and train the multilingual translation task by tuning it. To fully reserve the capacity of well-trained models, we do not change the architectures of BERT or GPT. Also, the tuning is mainly targeted at the parameters of the bridge.
Experiments show that our method significantly improve the results of MNMT and outperform previous works of both \textit{United Style} and \textit{Assembled Style}.



==> 010intro_v2.tex <==

Multilingual neural machine translation (MNMT) has recently become an important research field for the deployment efficiency and transfer learning for low-resource language pairs~\cite{aharoni2019massively}. Most related works follow~\newcite{johnson2017google} and train all language pairs together within a single model. It is proved that such mixed training can significantly improve the performance of low-resource pairs~\cite{arivazhagan2019massively}.

In bilingual NMT, incorporating pre-trained NLP models like BERT~\cite{devlin2019bert} and GPT~\cite{radford2018improving} with NMT has show its effect~\cite{yang2020towards,zhu2020incorporating,rothe2020leveraging}. The pre-training and fine-tuning style becomes an important alternative to take advantage of monolingual data~\cite{weng2020acquiring}. Some similar attempts on MNMT are also conducted~\cite{ma2020xlm,yang2020alternating}.

However, while these methods can load encoder parameters from BERT or GPT, dealing with the translation decoder is not naive~\cite{rothe2020leveraging}. Pre-trained models are usually (masked) language models. They predict the current token only by the internal context while the translation decoder has to capture the source context. Specifically, the decoder in NMT has a "cross-attention" sub-layer that plays a transduction role~\cite{bahdanau2015neural}, while pre-trained models have none. This mismatch between the generation models and conditional generation models makes the usage of pre-trained models pretty tricky.

Most related works try to avoid this problem by fusing the pre-trained model and extra injected cross-attention~\cite{rothe2020leveraging,ma2020xlm}. Specifically, they insert a cross-attention layer (with random initialization) into the pre-trained encoder or decoder and conduct overall fine-tuning.
% With such methods, they try to make the pre-trained models be assimilated by the whole model and acquire the translation ability at the same time. 
However, the overall tuning can raise the problem of "catastrophic forgetting"~\cite{goodfellow2013empirical,yang2020towards}. The pre-trained language knowledge may gradually fade away. Therefore, the potential of the pre-trained model is not fully activated. \newcite{guo2020incorporating} propose to inject an adapter sub-layer into each layer of the pre-trained model and freeze the original parameters, achieving improvements. However, they still transform the original model architecture. The entire capacity of the pre-trained models is still restricted as long as the architecture discrepancy exists.

In this paper, we mainly focus on this challenge: how to bridge the pre-trained NLP models like BERT+GPT without limiting their strengths. The main target is to link the generation model to the source side and maintain the invariability of the architecture at the same time. Therefore, we propose \textbf{GraftNet}, with pre-trained models grafted by a connective sub-module. The structure of the pre-trained parts remain unchanged and we train the grafting part to learn to translate.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/model_intro.pdf}
    \caption{Grafting pre-trained multilingual BERT and multilingual GPT to improve multilingual translation.}
    \label{fig:intro}
\end{figure}

Generally, the translation process can be divided into three parts: representation, transduction, and generation, respectively achieved by the encoder, cross-attention, and decoder. In MNMT, the transduciton can only be trained with multiple parallel data. But the rest two can be pre-trained with multiple monolingual data, which is tens or hundreds times of the parallel one. To maximize the efficacy of each part, we firstly pre-train a multilingual BERT and multilingual GPT. Then they are grafted to implement translation, as is in Figure~\ref{fig:intro}. With the architecture consistency, we can reserve the language knowledge of pre-trained models and obtain a strong translation model flexibly at the same time.

Experiments show that our method significantly improve the results of MNMT and outperform related works. The analysis also proves the importance of maintaining the well-trained ability of the generation model.


==> 010intro_v3.tex <==

% Multilingual neural machine translation (MNMT) has recently become an important research field for the deployment efficiency and transfer learning for low-resource language pairs~\cite{aharoni2019massively}. Most related works follow~\newcite{johnson2017google} and train all language pairs together within a single model. It is proved that such mixed training can significantly improve the performance of low-resource pairs~\cite{arivazhagan2019massively}.

In recent years, pre-trained models achieve significant progress in all kinds of NLP tasks~\cite{devlin2019bert,radford2019language}. Among them, combining with neural machine translation (NMT) is also explored by several attempts~\cite{yang2020towards,zhu2020incorporating,rothe2020leveraging}. The pre-training and fine-tuning style becomes an important alternative to take advantage of monolingual data~\cite{yang2020csp,yang2020alternating}.

However, though many works successfully gain improvements by loading encoder/decoder parameters from BERT-like pre-trained encoders~\cite{zhu2020incorporating,guo2020incorporating}, they do not achieve satisfactory results with loading decoder parameters from GPT-like pre-trained decoders~\cite{yang2020towards,rothe2020leveraging}. Theoretically, the well-trained decoder model like GPT should bring better generation ability to the translation model. We suggest the outcome may be attributed to the architecture mismatch. 


\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/model_intro.pdf}
    \caption{Taking the popular architecture Transformer~\cite{vaswani2017attention} as an example, the translation model has a ``cross-attention'' sub-layer, while pre-trained models have none.}
    \captionsetup{font={scriptsize}}
    \label{fig:intro}
\end{figure}

Pre-trained models are usually (masked) language models. They predict the current word only based on the internal context while the translation decoder has to capture the source context. Specifically, the decoder in NMT has a ``cross-attention'' sub-layer that plays a transduction role~\cite{bahdanau2015neural}, while pre-trained models have none, as is in Figure~\ref{fig:intro}. This mismatch between the generation models and conditional generation models makes the pre-trained model usage for translation decoder pretty tricky. 

Therefore, some previous works manually insert cross-attention sub-layer or adapters~\cite{rothe2020leveraging,ma2020xlm,guo2020incorporating}. However, the extra implantation may influence the ability of the pre-trained model. Other works try to avoid this problem by directly pre-training a seq2seq model and conduct fine-tuning~\cite{tang2020multilingual,yang2020alternating,luo2020veco}. However, the pre-training objective is usually a variant of auto-encoding~\cite{song2019mass,liu2020multilingual}, which is different from the downstream translation objective and may not achieve adequate improvements~\cite{lin2020pre}. 

In this paper, we mainly focus on exploring the best way to simultaneously take advantage of the pre-trained representation model and generation model (e.g., BERT+GPT) without limiting their strengths. The main target is to link the generation model to the source side and maintain the invariability of the architecture at the same time. Therefore, we propose \textbf{\model}, with pre-trained models grafted by a connective sub-module. The structure of the pre-trained parts remains unchanged, and we train the grafting part to learn to translate. For universality and generalization, we also extend the model to multilingual NMT, achieving mBERT+mGPT.

Generally, the translation process can be divided into three parts: representation, transduction, and generation, respectively achieved by the encoder, cross-attention, and decoder. In MNMT, the transduction can only be trained with multiple parallel data. But the rest two can be pre-trained with multiple monolingual data, which is tens or hundreds of the parallel one. To maximize the efficacy of each part, we firstly pre-train a multilingual BERT and multilingual GPT. Then they are grafted to implement translation. With the architecture consistency, we can reserve the language knowledge of the pre-trained models and obtain a strong translation model flexibly at the same time.

Experiments show that our method significantly improves the results of MNMT and outperforms related works. The analysis also proves the importance of maintaining the well-trained ability of the generation model.


==> 040experiments_backup.tex <==

\begin{table*}[ht]
    \centering
    \begin{tabular}{l|cccccccccc}
        \Xhline{3\arrayrulewidth}
        Model & bg & bn & bs & cs & de & el & es & et & fa & fi \\ \hline
        Baseline & 32.0 & 12.5 & 30.3 & 23.7 & 28.7 & 30.7 & 34.7 & 17.5 & 20.4 & 17.1 \\
        mBART & - & - & - & 26.4 & 32.8 & - & 38.1 & 20.9 & - & 19.9 \\
        % load & 36.8 & 18.0 & 35.2 & 28.5 & 33.9 & 35.3 & 39.1 & 22.5 & 24.8 & 21.2 \\
        \model & \textbf{38.5} & \textbf{18.1} & \textbf{36.5} & \textbf{29.4} & \textbf{35.5} & \textbf{37.4} & \textbf{40.7} & \textbf{24.0} & \textbf{26.9} & \textbf{23.0} \\
        \Xhline{3\arrayrulewidth}
        Model & fr & hi & hr & hu & it & ja & kk & lt & mk & mr \\ \hline
        Baseline & 33.1 & 18.7 & 30.4 & 19.8 & 31.3 & 10.1 & 7.6 & 20.1 & 29.8 & 9.4 \\
        mBART & 36.5 & 22.9 & - & - & 34.7 & 12.0 & 8.9 & 23.6 & - & - \\
        % load & 38.0 & 23.6 & 35.3 & 24.4 & 36.0 & 12.3 & 10.1 & 25.4 & 33.8 & 12.1 \\
        \model & \textbf{39.2} & \textbf{25.1} & \textbf{36.7} & \textbf{26.1} & \textbf{37.2} & \textbf{13.7} & \textbf{10.5} & \textbf{27.2} & \textbf{35.7} & \textbf{13.0} \\
        \Xhline{3\arrayrulewidth}
        Model & nl & pl & pt & ro & ru & sr & ta & tr & uk & zh \\ \hline
        Baseline & 28.9 & 19.7 & 34.8 & 28.6 & 20.8 & 29.0 & 5.8 & 18.7 & 23.4 & 15.6 \\
        mBART & 32.9 & - & - & 32.2 & 22.6 & - & - & 22.6 & - & 18.1 \\
        % load & 33.2 & 23.6 & 40.1 & 33.6 & 23.9 & 33.9 & 8.7 & 23.3 & 27.8 & 18.5 \\
        \model & \textbf{35.2} & \textbf{25.1} & \textbf{41.5} & \textbf{35.1} & \textbf{25.1} & \textbf{35.6} & \textbf{10.2} & \textbf{25.5} & \textbf{28.9} & \textbf{19.9} \\
        \Xhline{3\arrayrulewidth}
    \end{tabular}
    \caption{The results of x$\rightarrow$en directions, with average improvements of 5.8 against baseline (22.8$\rightarrow$28.6)}
    \label{tab:x2en}
\end{table*}

\begin{table*}[ht]
    \centering
    \begin{tabular}{l|cccccccccc}
        \Xhline{3\arrayrulewidth}
        Model & bg & bn & bs & cs & de & el & es & et & fa & fi \\ \hline
        Baseline & 28.8 & 11.3 & 23.4 & 16.6 & 23.7 & 25.9 & 33.0 & 14.0 & 12.5 & 12.1 \\
        mBART & - & - & - & 17.7 & 25.8 & - & 35.2 & 14.1 & - & 13.2 \\
        % load & 30.7 & 12.2 & 24.5 & 18.2 & 25.1 & 27.8 & 35.3 & 14.9 & 13.3 & 13.1 \\
        \model & \textbf{33.0} & \textbf{14.1} & \textbf{26.3} & \textbf{20.2} & \textbf{27.8} & \textbf{29.8} & \textbf{37.5} & \textbf{16.1} & \textbf{14.2} & \textbf{14.4} \\
        \Xhline{3\arrayrulewidth}
        Model & fr & hi & hr & hu & it & ja & kk & lt & mk & mr \\ \hline
        Baseline & 33.5 & 15.3 & 23.2 & 14.7 & 28.9 & 11.1 & 3.4 & 12.8 & 22.2 & 9.3 \\
        mBART & 35.8 & 16.5 & - & - & 30.6 & 12.6 & 3.0 & 14.2 & - & - \\
        % load & 35.4 & 16.7 & 25.2 & 15.7 & 30.7 & 12.2 & 4.0 & 14.5 & 24.4 & 10.5 \\
        \model & \textbf{37.8} & \textbf{18.1} & \textbf{26.8} & \textbf{17.2} & \textbf{32.5} & \textbf{12.8} & \textbf{3.8} & \textbf{15.9} & \textbf{25.7} & \textbf{10.6} \\
        \Xhline{3\arrayrulewidth}
        Model & nl & pl & pt & ro & ru & sr & ta & tr & uk & zh \\ \hline
        Baseline & 25.9 & 12.8 & 32.0 & 24.7 & 16.1 & 18.7 & 13.6 & 11.6 & 17.3 & 21.2 \\
        mBART & 28.9 & - & - & 27.1 & 16.9 & - & - & \textbf{13.4} & - & 22.2 \\
        % load & 28.1 & 14.4 & 34.3 & 26.9 & 17.5 & 20.2 & 15.6 & 12.3 & 18.7 & 21.8 \\
        \model & \textbf{29.0} & \textbf{15.8} & \textbf{36.6} & \textbf{29.1} & \textbf{19.0} & \textbf{21.4} & \textbf{14.7} & 13.3 & \textbf{19.5} & \textbf{23.0} \\
        \Xhline{3\arrayrulewidth}
    \end{tabular}
    \caption{The results of en$\rightarrow$x directions, with average improvements of 2.9 against baseline (19.0$\rightarrow$21.9)}
    \label{tab:en2x}
\end{table*}

In this paper, we perform many-to-many style multilingual translation~\cite{johnson2017google}. The detailed illustrations of the datasets and implementation are as follows.

\subsection{Datasets and Preprocess}
\begin{compactitem}
    \item \textbf{Pre-training:} We use News-Crawl corpus~\footnote{\url{http://data.statmt.org/news-crawl}} plus WMT datasets. We conduct deduplication and label the data by language. In the end, we collect 1.4 billion sentences in 45 languages, which is only one-fifth of that of mBART~\cite{liu2020multilingual}. The detailed list of languages and scales is in Appendix~\ref{apdx:langs}.
    \item \textbf{Multilingual Translation:} We use TED datasets, the most widely used MNMT datasets, following~\newcite{qi2018and,aharoni2019massively}. We extract 30 languages~\footnote{We use the corpus of ``zh\_cn'' instead of ``zh''.} from \& to English, with the size of 3.18M sentence pairs in raw data and 10.1M sentence pairs in sampled bidirectional data. The detailed list of language pairs and scales is in Appendix~\ref{apdx:langs}.
    We download the data from the open source~\footnote{\url{https://github.com/neulab/word-embeddings-for-nmt}} and conduct detokenization with Moses Detokenizer~\cite{koehn2007moses}~\footnote{\url{https://github.com/moses-smt/mosesdecoder/blob/master/scripts/tokenizer/detokenizer.perl}}.
    \item \textbf{Zero-shot and Bilingual Translation:} We use WMT 2014 German-English (4.5M sentence pairs) and French-English (36M sentence pairs) datasets.
    \item \textbf{Sample:} Upsampling is an important way to improve the performance of low-resource pairs~\cite{arivazhagan2019massively}. Therefore, sentences are sampled according to a multinomial distribution with probabilities $\{q_i\}$, where $q_i \propto p_i^{\alpha}$, $p_i$ is the proportion of language$_i$.
    For monolingual pre-training, we follow~\cite{conneau2019cross,liu2020multilingual} and set $\alpha=0.7$. For parallel fine-tuning, we follow~\cite{arivazhagan2019massively} and and set $\alpha=0.2$ ($T=5$).
    \item \textbf{Tokenization:} Like previous works, we use sentencepiece~\cite{kudo2018sentencepiece} and learn a joint vocabulary of 64000 tokens.
\end{compactitem}

\subsection{Implementation Details}

\begin{compactitem}
    \item \textbf{Architecture:} We use Transformer~\cite{vaswani2017attention} as our basic structure with pre-norm style~\cite{xiong2020layer}, and GLUE~\cite{hendrycks2016gaussian} as activation function. Specifically, we adopt 1024 dimensions for the hidden state, 4096 dimensions for the middle FFN layer, and 16 heads for multi-head attention. Learnable position embedding is also employed. For baseline models, we use 12 layers. For pre-trained ones, we use Transformer encoder and decoder (without cross-attention) with 6 layers, respectively. For the grafting part, we add another 6 layers.
    \item \textbf{Training:} We train the models with a batch size of 320,000 tokens on 16 Tesla V100 GPUs. For pre-training, we go through the total data for five times. Parameters are optimized by using Adam optimizer~\cite{kingma2015adam}, with $\beta_1=0.9$, $\beta_2=0.98$, with $warmup\_steps=4000$. Without extra statement, we use dropout $=0.3$~\cite{srivastava2014dropout}. Label smoothing \cite{szegedy2016rethinking} of value $=0.1$ is also adopted. Besides, we use fp16 mixed precision training~\cite{micikevicius2018mixed} with Horovod library with RDMA inter-GPU communication~\cite{sergeev2018horovod}. 
    \item \textbf{Evaluation:} We uniformly conduct beam search with size $=5$ and length penalty $\alpha=0.6$. For hi, ja, and zh, we use SacreBLEU~\cite{post2018call}. Otherwise, we use tokenized BLEU~\cite{papineni2002bleu} with the open-source script~\footnote{\url{https://github.com/pytorch/fairseq/blob/master/examples/m2m_100/tok.sh}}.
\end{compactitem}

\subsection{Main Results}

As is shown in Table~\ref{tab:x2en} and \ref{tab:en2x}, our methods obtain significant improvements across all language pairs. For x$\rightarrow$en and en$\rightarrow$x pairs, advances of nearly 6 BLEU and 3 BLEU are achieved. We also compare the results with loading from mBART, a well-known multilingual pre-trained sequence-to-sequence model~\cite{liu2020multilingual}~\footnote{\url{https://dl.fbaipublicfiles.com/fairseq/models/mbart/mbart.cc25.v2.tar.gz}}. Due to the language difference, we only tune the model on a part of languages. With both 12-layers depth and 1024-dimensions width, our method outperforms mBART on almost all pairs, proving the superiority of \model comparing with pre-training in United Style mentioned in Section~\ref{sec:related}.

\subsection{Ablation Study}

To verify the contribution of each part of our model, we do a series of ablation studies. As is shown in Table~\ref{tab:ablation}, we can draw at least three empirical conclusions.

\textbf{Encoder needs tuning, decoder needs not.} Comparing Row 1 with Row 2, and Row 5 with Row 8, we can see that the tuning of the encoder is essential. It can bring further improvements. However, freezing pre-trained decoder parameters is a better choice. Comparing Row 3 with Row 4, and Row 6 with Row 8, we can see that tuning may lead to a drop for decoder. It seems that the pre-trained decoder model learns much more knowledge, and its original language model can better guide the generation.

\textbf{Decoder matters more.} Comparing Row 1,2,3,4, we can see that the pre-trained decoder yields more progress than the pre-trained encoder. This shows that involving only pre-trained encoders like BERT into MT is limited. The performance can be further enhanced with the introduction of pre-trained decoders.

\textbf{Residual connection contributes.} Comparing Row 7 with Row 8, we can see that the residual connection from the pre-trained decoder can further boost the results. The well-trained language model effectively helps the translation model. It also shows the importance of incorporating the knowledge-rich generation model.

\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|cc}
        \Xhline{3\arrayrulewidth}
        Row & Encoder & Decoder & x$\rightarrow$en & en$\rightarrow$x \\
        \Xhline{3\arrayrulewidth}
        0 & - & - & 22.8 & 19.0 \\
        1 & Freeze	& -	& 23.2 & 19.2 \\
        2 & Fine-tune & - & 27.0 & 20.2 \\
        3 & - & Freeze & 27.8 & 21.0 \\
        4 & - & Fine-tune & 25.2 & 19.9 \\
        5 & Freeze & Freeze & 25.8 & 20.4 \\
        6 & Fine-tune & Fine-tune & 27.0 & 19.4 \\
        7 & Fine-tune & Freeze* & 28.1 & 20.9 \\
        8 & Fine-tune & Freeze & \textbf{28.6} & \textbf{21.9} \\
        \Xhline{3\arrayrulewidth}
    \end{tabular}
    % \captionsetup{font={footnotesize}}
    \caption{Each number is the average BLEU of 30 language directions. ``-'' means not loading from pre-trained models. ``*'' means the residual connection is abandoned.}
    \label{tab:ablation}
\end{table}
\subsection{Well-trained Language Model Helps}

Except for BLEU, we also study how the pre-trained generation model influence the translation model. We speculate that the pre-trained decoder helps to translate through combining the well-trained language model. Therefore, we measure the perplexity of the models on the validation sets.

As is in Table~\ref{tab:ppl}, we can see that our method significantly lowers the perplexity comparing to the baseline model. The pre-trained decoder brings in better representation and language knowledge. Also, the residual connection from the original pre-trained decoder can further improve the results, illustrating the enlightening role the well-trained language model plays.

\begin{table}[h]
    \centering
    \begin{tabular}{l|cc}
        \Xhline{3\arrayrulewidth}
        Model & x$\rightarrow$en & en$\rightarrow$x \\
        \hline
        Baselne & 8.64 & 8.76 \\
        \model* & 5.60 & 6.58 \\
        \model & \textbf{5.27} & \textbf{6.21} \\
        \Xhline{3\arrayrulewidth}
    \end{tabular}
    % \captionsetup{font={footnotesize}}
    \caption{The perplexity of models. Each number is the average result of 30 language directions. ``*'' means the residual connection is abandoned.}
    \label{tab:ppl}
\end{table}

\subsection{Better than Fused Styles}

Besides \textit{United Style} (mBART), we also compare our method with \textit{Fused Style}. Specifically, we choose two typical works, as are in Figure~\ref{fig:others}: \textit{1)} loading parameters directly and ignoring cross-attention (denoted as ``Direct'')~\cite{rothe2020leveraging,ma2020xlm}; \textit{2)} insert extra cross-attention layers into each decoder sub-layer and freeze pre-trained models (denoted as ``Adapter'')~\cite{guo2020incorporating}. We re-implement the models with the same depth and width as \model.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/model_load.pdf}
%     \caption{The model architecture of~\newcite{rothe2020leveraging,ma2020xlm}: directly loading the parameters of the pre-trained encoder and decoder (except cross-attention) and tuning all.}
%     \captionsetup{font={footnotesize}}
%     \label{fig:load}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/model_ab.pdf}
%     \caption{The model architecture of~\newcite{guo2020incorporating}: insert extra cross-attention layers into each decoder sub-layer and freeze pre-trained models.}
%     \captionsetup{font={footnotesize}}
%     \label{fig:ab}
% \end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/model_others.pdf}
    \caption{The model architecture of ``Direct'' (left)~\cite{rothe2020leveraging,ma2020xlm} and ``Adapter'' (right)~\cite{guo2020incorporating}.}
    % \captionsetup{font={footnotesize}}
    \label{fig:others}
\end{figure}

\begin{table}[h]\footnotesize
    \centering
    \begin{tabular}{l|cc|cc}
        \Xhline{3\arrayrulewidth}
        \multirow{2}{*}{Model} & \multicolumn{2}{c|}{BLEU$\uparrow$} & \multicolumn{2}{c}{Perplexity$\downarrow$} \\ 
        \cline{2-5}
        & x$\rightarrow$en & en$\rightarrow$x & x$\rightarrow$en & en$\rightarrow$x \\ 
        \hline
        Direct & 27.1 & 20.5 & 6.61 & 8.06 \\ 
        Adapter & 27.4 & 19.8 & 5.78 & 6.71 \\
        \model & \textbf{28.6} & \textbf{21.9} & \textbf{5.27} & \textbf{6.21} \\
        \Xhline{3\arrayrulewidth}
    \end{tabular}
    \caption{Each number is the average BLEU/Perplexity of 30 language directions. Our model
    outperform related methods in fused style.}
    \label{tab:model}
\end{table}

As is in Table~\ref{tab:model}, our approach outperforms other two methods (The detailed results are in Appendix~\ref{apdx:assembled}). The crucial difference is that we leave the pre-trained decoder module unchanged and complete. However, other works inject extra layers internally, such as cross-attention or adapters. No matter tuned or not, the architecture is inconsistent with the one in the pre-trained stage, which can not activate the full potential of the pre-trained decoder. Differently, we maintain the original structure and even feed its output into the final layer. These strategies are all for the sake of fully taking advantage of the pre-trained generation model.

\subsection{\model Maintains Good Performance in Few-Shot Translation}

We also conduct few-shot experiments. We randomly select 30\%, 10\%, 3\%, 1\% of the data and reproduce the experiments. As is in Figure~\ref{fig:x2en},\ref{fig:en2x}, as the scale of datasets decreases, the performance of baseline drops dramatically and fails to generate comprehensible sentences (BLEU < 5). However, our method keeps relatively higher results even with only 1\% data. And with the less data provided, the gap between \model and baseline is much larger (5.8$\rightarrow$12.1, 2.9$\rightarrow$7.1). Again, it proves that the usage of multiple monolingual data can benefit MNMT greatly since its scale is tens or hundreds of times of the parallel one.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.495\textwidth]{figures/few_x2en.pdf}
    \caption{The results of x$\rightarrow$en directions. As the data scale decrease from 100\% to 1\%, the gap is getting larger (5.8$\rightarrow$12.1).}
    \label{fig:x2en}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.495\textwidth]{figures/few_en2x.pdf}
    \caption{The results of en$\rightarrow$x directions. As the data scale decrease from 100\% to 1\%, the gap is getting larger (2.9$\rightarrow$7.1).}
    \label{fig:en2x}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.495\textwidth]{figures/bleu.pdf}
    \caption{Each point represents a language. The x-axis means the quotient of the monolingual data scale divided by the parallel data scale. The y-axis means the BLEU improvements of en$\rightarrow$x directions.}
    \label{fig:bleu}
\end{figure}

\subsection{The More Monolingual data, The Better}

To further analyze the effectiveness of monolingual data, we look into the relationship between the BLEU advance and the data scale. As is in Figure~\ref{fig:bleu}, as the quotient of the monolingual data scale divided by the parallel data scale increases, the BLEU improvements gradually go up. It shows the extra benefit provided by the monolingual data, especially in the large-scale scene. Since the parallel data is sparse and rare, \model can be an essential approach to enhance low-resource language pairs.

\subsection{\model Boosts Zero-Shot Translation}

To verify whether the multilingual pre-trained model learns cross-lingual knowledge, we also conduct a crossed experiment of zero-shot translation. Firstly, we use our approach to train models only on German-English corpus and then conduct inference on French-English test sets. Converse ones are done similarly. We perform experiments on both TED and WMT datasets, with the encoder frozen ($\text{\model}_{fe}$) and tuned (\model).

\begin{table}[h]
    \centering
    \begin{tabular}{c|l|cc}
        \Xhline{3\arrayrulewidth}
        \multirow{2}{*}{Train} & 
        \multirow{2}{*}{Model} & \multicolumn{2}{c}{Testing} \\ 
        \cline{3-4} 
        &  & de$\rightarrow$en & fr$\rightarrow$en \\ 
        \hline
        \multirow{3}{*}{de$\rightarrow$en} & baseline & 31.9 & 6.7 \\ 
         & \model & \textbf{33.4} & 15.2 \\ 
         & $\text{\model}_{fe}$ & 33.0 & \textbf{20.1} \\ 
        \hline
        \multirow{3}{*}{fr$\rightarrow$en} & baseline & 5.1 & 35.1 \\ 
         & \model & 10.8 & \textbf{36.0} \\
         & $\text{\model}_{fe}$ & \textbf{16.8} & 35.5  \\
         \Xhline{3\arrayrulewidth}
    \end{tabular}
    \caption{Zero-shot experiments on WMT Datasets. ``$fe$'' means freezing the pre-trained encoder.}
    \label{tab:zero_wmt}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{c|l|cc}
        \Xhline{3\arrayrulewidth}
        \multirow{2}{*}{Train} & 
        \multirow{2}{*}{Model} & \multicolumn{2}{c}{Testing} \\ 
        \cline{3-4} 
        &  & de$\rightarrow$en & fr$\rightarrow$en \\ 
        \hline
        \multirow{3}{*}{de$\rightarrow$en} & baseline & 33.6 & 1.7 \\ 
         & \model & \textbf{36.9} & 3.4 \\ 
         & $\text{\model}_{fe}$ & 35.4 & \textbf{11.9} \\ 
        \hline
        \multirow{3}{*}{fr$\rightarrow$en} & baseline & 1.5 & 37.3 \\ 
         & \model & 4.5 & \textbf{40.7} \\
         & $\text{\model}_{fe}$ & \textbf{10.7} & 39.8 \\
         \Xhline{3\arrayrulewidth}
    \end{tabular}
    \caption{Zero-shot experiments on TED Datasets. $``fe''$ means freezing the pre-trained encoder.}
    \label{tab:zero_ted}
\end{table}

As is in Table~\ref{tab:zero_wmt} and \ref{tab:zero_ted}, we can draw similar conclusions. On the one hand, the performance of the original direction is improved, as expected. On the other hand, the inference results in the other direction are also significantly boosted. It is worth noting that our models are trained with none of the test directions but obtain BLEU score high than 10.

More specifically, if the encoder is frozen, the results of the main direction can be slightly lowered, but the results of the zero-shot one will be significantly improved. It illustrates that the untuned pre-trained model contains much more cross-lingual knowledge and can be better transferred to untrained pairs.

\subsection{\model Works in Bilingual Translation}

To verify the effect of our methods, we also conduct experiments on bilingual translation. We use WMT14  English-German and English-French Datasets. In this setting, the datasets and vocabulary of both pre-training and tuning are limited in bilingual corpus. For en-fr training, we use dropout=0.1, following~\newcite{vaswani2017attention}. The results, along with several strong related pre-training works, are listed in Table~\ref{tab:bilingual}. They all take advantage of pre-trained models and significantly improve the translation. Our method boosts the performance of bilingual translation and is at the top level. It proves the universal effectiveness of \model.

\begin{table}[ht]
    \centering
    \begin{tabular}{l|cc}
        \Xhline{3\arrayrulewidth}
        Model & en$\rightarrow$de & en$\rightarrow$fr \\
        \hline
        Baseline & 28.9 & 41.8 \\
        \newcite{yang2020towards} & 30.1 & 42.3 \\
        \newcite{weng2020acquiring} & 29.2 & - \\
        \newcite{yang2020alternating} & 29.2 & - \\
        \newcite{zhu2020incorporating} & 30.8 & \textbf{43.8} \\
        \newcite{rothe2020leveraging} & 30.6 & - \\
        \newcite{guo2020incorporating} & 30.6 & 43.6 \\
        \hline
        \model & \textbf{31.0} & 43.6 \\
        \Xhline{3\arrayrulewidth}
    \end{tabular}
    \caption{Bilingual translation results of English-German and English-French of WMT14. Comparing objects are strong results reported by recent works. \model boosts the performance and is at the top level.}
    \label{tab:bilingual}
\end{table}

% \subsection{Speed Analysis}

% \begin{table}[ht]
%     \centering
%     \begin{tabular}{l|c}
%         \Xhline{3\arrayrulewidth}
%         Model & Training speed \\
%         \hline
%         Baseline & 1.00 \\
%         $\text{\model}_{freeze\_enc}$ & $\times$1.53 \\
%         \model & $\times$1.21 \\
%         \Xhline{3\arrayrulewidth}
%     \end{tabular}
%     \caption{The training speed comparison between \model and Baseline. With}
%     \label{tab:speed}
% \end{table}

